Diversity and Generalization in Neural Network Ensembles

Ensembles are widely used in machine learning and, usually, provide state-of-the-art performance in many prediction tasks. From the very beginning, the diversity of an ensemble has been identified as a key factor for the superior performance of these models. But the exact role that diversity plays in ensemble models is poorly understood, specially in the context of neural networks. In this work, we combine and expand previously published results in a theoretically sound framework that describes the relationship between diversity and ensemble performance for a wide range of ensemble methods. More precisely, we provide sound answers to the following questions: how to measure diversity, how diversity relates to the generalization error of an ensemble, and how diversity is promoted by neural network ensemble algorithms. This analysis covers three widely used loss functions, namely, the squared loss, the cross-entropy loss, and the 0-1 loss; and two widely used model combination strategies, namely, model averaging and weighted majority vote. We empirically validate this theoretical analysis with neural network ensembles.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{All assumptions are stated in the statements of the theorems.} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{In Section 7.} 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Section 6 and in Appendix F.} 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Section 6 and in Appendix F.} 
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} In Appendix F.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} In the code and in the paper.
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} New code in the supplementary.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{} We use publicly available datasets.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{} We use publicly available datasets. The data does not contain personally identifiable information or offensive content.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> hl_short.tex <==
\usepackage{xspace}
\usepackage{graphics,graphicx,epsfig}
\usepackage{url}

\newcommand{\nc}{\newcommand}

%      HELGE's EGNE "NEWCOMMANDS"



%%      THEOREMER OG SLIKT%
%
\newtheorem{hl_example}{Example}
\newtheorem{hl_algorithm}{Algorithm}
\newtheorem{hl_theorem}{Theorem}
\newtheorem{hl_proposition}{Proposition}
\newtheorem{hl_lemma}{Lemma}
\newtheorem{hl_corollary}{Corollary}
\newtheorem{hl_definition}{Definition}
\newtheorem{hl_conjecture}{Conjecture}
\newenvironment{hl_nonumberenv}[1]{{\bf #1}\begin{it}}{\end{it}}
\newtheorem{hl_proof}{Proof}



%      KOMMENTARMARKERING

\nc{\vekk}[1]{}   %         \vekk{Brukes for � markere vekk tekst}
%\nc{\comment}[1]{\mbox{}\marginpar{\raggedright\hspace{0pt}#1}}%
%\nc{\hl}[1]{\comment{{\bf HL:} #1}} %
\nc{\tdn}[1]{\comment{{\bf TDN:} #1}} %



%      BEGIN/END

\nc{\bex}{\begin{example}} \nc{\eex}{\end{example}}

%\nc{\bth}{\begin{theorem}}
%\nc{\eth}{\end{theorem}}

\nc{\ble}{\begin{lemma}}
\nc{\ele}{\end{lemma}}

\nc{\bco}{\begin{conjecture}}
\nc{\eco}{\end{conjecture}}

\nc{\beq}{\begin{equation}}
\nc{\eeq}{\end{equation}}

\nc{\beqa}{\begin{eqnarray}}
\nc{\eeqa}{\end{eqnarray}}

\nc{\beqas}{\begin{eqnarray*}}%
\nc{\eeqas}{\end{eqnarray*}}

\nc{\bsp}{\[\begin{array}{rcl}}
\nc{\esp}{\end{array}\]}

\nc{\btab}[1]{\begin{tabular}{#1}}
\nc{\etab}{\end{tabular}}

\nc{\bfi}{\begin{figure}[htpb]}
\nc{\efi}{\end{figure}}

\nc{\ben}{\begin{enumerate}}
\nc{\een}{\end{enumerate}}

\nc{\bit}{\begin{itemize}}
\nc{\eit}{\end{itemize}}

\nc{\bde}{\begin{description}}
\nc{\ede}{\end{description}}


%      PRODUKT, BINOMISKE TING OG SUMMER

\nc{\pin}{\prod_{i=1}^n} \nc{\pjm}{\prod_{j=1}^m}
\nc{\pkm}{\prod_{k=1}^m} \nc{\pjM}{\prod_{j=1}^M}
\nc{\suin}{\sum_{i=1}^n} \nc{\sujm}{\sum_{j=1}^m}
\nc{\sukm}{\sum_{k=1}^m} \nc{\sujM}{\sum_{j=1}^M} \nc{\bimr}{\left
(_r^m \right)} \nc{\birs}{\left (_s^r \right)}
\nc{\bin}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      CAL-TING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\nc{\cal}{\mathcal}

\nc{\calDelta}{\mbox{$\cal{\Delta}$}}

% \nc{\calA}{\mbox{${\cal A}$}} \nc{\calB}{\mbox{$\cal{B}$}}
% \nc{\calC}{\mbox{$\cal{C}$}} \nc{\calD}{\mbox{$\cal{D}$}}
% \nc{\calE}{\mbox{$\cal{E}$}} \nc{\calF}{\mbox{$\cal{F}$}}
% \nc{\calG}{\mbox{$\cal{G}$}} \nc{\calH}{\mbox{$\cal{H}$}}
% \nc{\calI}{\mbox{$\cal{I}$}} \nc{\calJ}{\mbox{$\cal{J}$}}
% \nc{\calK}{\mbox{$\cal{K}$}} \nc{\calL}{\mbox{$\cal{L}$}}
% \nc{\calM}{\mbox{$\cal{M}$}} \nc{\calN}{\mbox{$\cal{N}$}}
% \nc{\calO}{\mbox{$\cal{O}$}} \nc{\calP}{\mbox{$\cal{P}$}}
% \nc{\calQ}{\mbox{$\cal{Q}$}} \nc{\calR}{\mbox{$\cal{R}$}}
% \nc{\calS}{\mbox{$\cal{S}$}} \nc{\calT}{\mbox{$\cal{T}$}}
% \nc{\calU}{\mbox{$\cal{U}$}} \nc{\calV}{\mbox{$\cal{V}$}}
% \nc{\calW}{\mbox{$\cal{W}$}} \nc{\calX}{\mbox{$\cal{X}$}}
% \nc{\calY}{\mbox{$\cal{Y}$}} \nc{\calZ}{\mbox{$\cal{Z}$}}
% \nc{\calz}{\mbox{$\cal{z}$}}



\nc{\calA}{{\ensuremath{\cal{A}}}} \nc{\calB}{{\ensuremath{\cal{B}}}}
\nc{\calC}{{\ensuremath{\cal{C}}}} \nc{\calD}{{\ensuremath{\cal{D}}}}
\nc{\calE}{{\ensuremath{\cal{E}}}} \nc{\calF}{{\ensuremath{\cal{F}}}}
\nc{\calG}{{\ensuremath{\cal{G}}}} \nc{\calH}{{\ensuremath{\cal{H}}}}
\nc{\calI}{{\ensuremath{\cal{I}}}} \nc{\calJ}{{\ensuremath{\cal{J}}}}
\nc{\calK}{{\ensuremath{\cal{K}}}} \nc{\calL}{{\ensuremath{\cal{L}}}}
\nc{\calM}{{\ensuremath{\cal{M}}}} \nc{\calN}{{\ensuremath{\cal{N}}}}
\nc{\calO}{{\ensuremath{\cal{O}}}} \nc{\calP}{{\ensuremath{\cal{P}}}}
\nc{\calQ}{{\ensuremath{\cal{Q}}}} \nc{\calR}{{\ensuremath{\cal{R}}}}
\nc{\calS}{{\ensuremath{\cal{S}}}} \nc{\calT}{{\ensuremath{\cal{T}}}}
\nc{\calU}{{\ensuremath{\cal{U}}}} \nc{\calV}{{\ensuremath{\cal{V}}}}
\nc{\calW}{{\ensuremath{\cal{W}}}} \nc{\calX}{{\ensuremath{\cal{X}}}}
\nc{\calY}{{\ensuremath{\cal{Y}}}} \nc{\calZ}{{\ensuremath{\cal{Z}}}}
\nc{\calz}{{\ensuremath{\cal{z}}}}



%\nc{\NP}{\mbox{$\calN\calP$}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      BOLDMATH-TING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\bm}{\boldmath}
% \nc{\bm}{\bf}
\nc{\bma}{{\ensuremath{\boldsymbol{a}}}} 
\nc{\bmb}{{\ensuremath{\boldsymbol{b}}}}
\nc{\bmc}{{\ensuremath{\boldsymbol{c}}}} \nc{\bmd}{{\ensuremath{\boldsymbol{d}}}}
\nc{\bme}{{\ensuremath{\boldsymbol{e}}}} \nc{\bmf}{{\ensuremath{\boldsymbol{f}}}}
\nc{\bmg}{{\ensuremath{\boldsymbol{g}}}} \nc{\bmh}{{\ensuremath{\boldsymbol{h}}}}
\nc{\bmi}{{\ensuremath{\boldsymbol{i}}}} \nc{\bmj}{{\ensuremath{\boldsymbol{j}}}}
\nc{\bmk}{{\ensuremath{\boldsymbol{k}}}} \nc{\bml}{{\ensuremath{\boldsymbol{l}}}}
\nc{\bmm}{{\ensuremath{\boldsymbol{m}}}} \nc{\bmn}{{\ensuremath{\boldsymbol{n}}}}
\nc{\bmo}{{\ensuremath{\boldsymbol{o}}}} \nc{\bmp}{{\ensuremath{\boldsymbol{p}}}}
\nc{\bmq}{{\ensuremath{\boldsymbol{q}}}} \nc{\bmr}{{\ensuremath{\boldsymbol{r}}}}
\nc{\bms}{{\ensuremath{\boldsymbol{s}}}} \nc{\bmt}{{\ensuremath{\boldsymbol{t}}}}
\nc{\bmu}{{\ensuremath{\boldsymbol{u}}}} \nc{\bmv}{{\ensuremath{\boldsymbol{v}}}}
\nc{\bmw}{{\ensuremath{\boldsymbol{w}}}} \nc{\bmx}{{\ensuremath{\boldsymbol{x}}}}
\nc{\bmy}{{\ensuremath{\boldsymbol{y}}}} \nc{\bmz}{{\ensuremath{\boldsymbol{z}}}}

% \nc{\bma}{{\mbox{\bm $a$}}} 
% \nc{\bmb}{{\mbox{\bm $b$}}}
% \nc{\bmc}{{\mbox{\bm $c$}}} \nc{\bmd}{{\mbox{\bm $d$}}}
% \nc{\bme}{{\mbox{\bm $e$}}} \nc{\bmf}{{\mbox{\bm $f$}}}
% \nc{\bmg}{{\mbox{\bm $g$}}} \nc{\bmh}{{\mbox{\bm $h$}}}
% \nc{\bmi}{{\mbox{\bm $i$}}} \nc{\bmj}{{\mbox{\bm $j$}}}
% \nc{\bmk}{{\mbox{\bm $k$}}} \nc{\bml}{{\mbox{\bm $l$}}}
% \nc{\bmm}{{\mbox{\bm $m$}}} \nc{\bmn}{{\mbox{\bm $n$}}}
% \nc{\bmo}{{\mbox{\bm $o$}}} \nc{\bmp}{{\mbox{\bm $p$}}}
% \nc{\bmq}{{\mbox{\bm $q$}}} \nc{\bmr}{{\mbox{\bm $r$}}}
% \nc{\bms}{{\mbox{\bm $s$}}} \nc{\bmt}{{\mbox{\bm $t$}}}
% \nc{\bmu}{{\mbox{\bm $u$}}} \nc{\bmv}{{\mbox{\bm $v$}}}
% \nc{\bmw}{{\mbox{\bm $w$}}} \nc{\bmx}{{\mbox{\bm $x$}}}
% \nc{\bmy}{{\mbox{\bm $y$}}} \nc{\bmz}{{\mbox{\bm $z$}}}


\nc{\bmA}{{\ensuremath{\boldsymbol{A}}}} \nc{\bmB}{{\ensuremath{\boldsymbol{B}}}}
\nc{\bmC}{{\ensuremath{\boldsymbol{C}}}} \nc{\bmD}{{\ensuremath{\boldsymbol{D}}}}
\nc{\bmE}{{\ensuremath{\boldsymbol{E}}}} \nc{\bmF}{{\ensuremath{\boldsymbol{F}}}}
\nc{\bmG}{{\ensuremath{\boldsymbol{G}}}} \nc{\bmH}{{\ensuremath{\boldsymbol{H}}}}
\nc{\bmI}{{\ensuremath{\boldsymbol{I}}}} \nc{\bmJ}{{\ensuremath{\boldsymbol{J}}}}
\nc{\bmK}{{\ensuremath{\boldsymbol{K}}}} \nc{\bmL}{{\ensuremath{\boldsymbol{L}}}}
\nc{\bmM}{{\ensuremath{\boldsymbol{M}}}} \nc{\bmN}{{\ensuremath{\boldsymbol{N}}}}
\nc{\bmO}{{\ensuremath{\boldsymbol{O}}}} \nc{\bmP}{{\ensuremath{\boldsymbol{P}}}}
\nc{\bmQ}{{\ensuremath{\boldsymbol{Q}}}} \nc{\bmR}{{\ensuremath{\boldsymbol{R}}}}
\nc{\bmS}{{\ensuremath{\boldsymbol{S}}}} \nc{\bmT}{{\ensuremath{\boldsymbol{T}}}}
\nc{\bmU}{{\ensuremath{\boldsymbol{U}}}} \nc{\bmV}{{\ensuremath{\boldsymbol{V}}}}
\nc{\bmW}{{\ensuremath{\boldsymbol{W}}}} \nc{\bmX}{{\ensuremath{\boldsymbol{X}}}}
\nc{\bmY}{{\ensuremath{\boldsymbol{Y}}}} \nc{\bmZ}{{\ensuremath{\boldsymbol{Z}}}}

% \nc{\bmA}{{\mbox{\bm $A$}}} \nc{\bmB}{{\mbox{\bm $B$}}}
% \nc{\bmC}{{\mbox{\bm $C$}}} \nc{\bmD}{{\mbox{\bm $D$}}}
% \nc{\bmE}{{\mbox{\bm $E$}}} \nc{\bmF}{{\mbox{\bm $F$}}}
% \nc{\bmG}{{\mbox{\bm $G$}}} \nc{\bmH}{{\mbox{\bm $H$}}}
% \nc{\bmI}{{\mbox{\bm $I$}}} \nc{\bmJ}{{\mbox{\bm $J$}}}
% \nc{\bmK}{{\mbox{\bm $K$}}} \nc{\bmL}{{\mbox{\bm $L$}}}
% \nc{\bmM}{{\mbox{\bm $M$}}} \nc{\bmN}{{\mbox{\bm $N$}}}
% \nc{\bmO}{{\mbox{\bm $O$}}} \nc{\bmP}{{\mbox{\bm $P$}}}
% \nc{\bmQ}{{\mbox{\bm $Q$}}} \nc{\bmR}{{\mbox{\bm $R$}}}
% \nc{\bmS}{{\mbox{\bm $S$}}} \nc{\bmT}{{\mbox{\bm $T$}}}
% \nc{\bmU}{{\mbox{\bm $U$}}} \nc{\bmV}{{\mbox{\bm $V$}}}
% \nc{\bmW}{{\mbox{\bm $W$}}} \nc{\bmX}{{\mbox{\bm $X$}}}
% \nc{\bmY}{{\mbox{\bm $Y$}}} \nc{\bmZ}{{\mbox{\bm $Z$}}}




\nc{\bmUpsilon}{{\mbox{\bm $\boldsymbol{\Upsilon}$}}}
\nc{\bmupsilon}{{\mbox{\bm $\boldsymbol{\upsilon}$}}}
\nc{\bmalpha}{{\mbox{\bm $\boldsymbol{\alpha}$}}}
\nc{\bmbeta}{{\mbox{\bm $\boldsymbol{\beta}$}}}
\nc{\bmgamma}{{\mbox{\bm $\boldsymbol{\gamma}$}}}
\nc{\bmGamma}{{\mbox{\bm $$\boldsymbol{\Gamma}$}}}
\nc{\bmdelta}{{\mbox{\bm $\boldsymbol{\delta}$}}}
\nc{\bmDelta}{{\mbox{\bm $\boldsymbol{\Delta}$}}}
\nc{\bmeps}{{\mbox{\bm $\boldsymbol{\epsilon}$}}}
\nc{\bmepsilon}{\bmeps}
\nc{\bmphi}{{\mbox{\bm $\boldsymbol{\phi}$}}}
\nc{\bmPhi}{{\mbox{\bm $\$\boldsymbol{\Phi}$}}}
\nc{\bmlambda}{{\mbox{\bm $\boldsymbol{\lambda}$}}}
\nc{\bmLambda}{{\mbox{\bm $\boldsymbol{\Lambda}$}}}
\nc{\bmmu}{{\mbox{\bm $\boldsymbol{\mu}$}}}
\nc{\bmnu}{{\mbox{\bm $\boldsymbol{\nu}$}}}
\nc{\bmpi}{{\mbox{\bm $\boldsymbol{\pi}$}}}
\nc{\bmrho}{{\mbox{\bm$\boldsymbol{\rho}$}}}
\nc{\bmpsi}{{\mbox{\bm $\boldsymbol{\psi}$}}}
\nc{\bmPsi}{{\mbox{\bm $\boldsymbol{\Psi}$}}}
\nc{\bmsigma}{{\mbox{\bm $$\boldsymbol{\sigma}$}}}
\nc{\bmSigma}{{\mbox{\bm $\boldsymbol{\Sigma}$}}}
\nc{\bmtheta}{{\ensuremath{\boldsymbol{\theta}}}}
%\nc{\bmTheta}{{\mbox{\bm $\Theta$}}}
\nc{\bmTheta}{{\ensuremath{\boldsymbol{\Theta}}}}
\nc{\bmeta}{{\ensuremath{\boldsymbol{\eta}}}}
\nc{\bmzeta}{{\mbox{\bm $\zeta$}}}
\nc{\bmxi}{{\mbox{\bm $\xi$}}} \nc{\bmXi}{{\mbox{\bm $\Xi$}}}
\nc{\bmnabla}{{\mbox{\bm $\nabla$}}}
\nc{\bmomega}{{\mbox{\bm $\omega$}}}
\nc{\bmOmega}{{\mbox{\bm $\Omega$}}}

\nc{\bmen}{{\bf 1}} \nc{\bmhalf}{{\bf\frac{1}{2}}}
\nc{\bmnull}{{\bf \ensuremath{0}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General terminology
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nc{\Var}{\mbox{Var}} \nc{\Cov}{\mbox{Cov}}
\nc{\E}{\mbox{$\mathbb{E}$}}
\nc{\KL}[2]{D\left(\,#1\,\norm\,#2\,\right)}
\nc{\convL}{\stackrel{\calL}{\rightarrow}} \nc{\given}{|}
%\nc{\norm}{||}
\nc{\norm}{\|} \nc{\sizeof}[1]{\left|#1\right|}

\nc{\iffp}{\mbox{$\Leftrightarrow$}} \nc{\ien}{\mbox{$i=1\ld n$}}
%\nc{\R}{\mbox{$\mathbb{R}$}}
\nc{\nat}{\mbox{$\mathbb{N}$}} \nc{\infinity}{\infty}
\nc{\ld}{,\ldots,} \nc{\defi}{:=} \nc{\incl}{\subset}
\nc{\upin}[2]{#1^{(#2)}} \nc{\non}{\nonumber}
\nc{\stless}{\stackrel{\mbox{st}}{\leq}}
\gdef\qed{\relax\ifmmode~\hfill\square\else\unskip\nobreak
    ~\hfill$\square$\fi}
\nc{\boxen}{\begin{flushright}$\rule{3mm}{3mm}$\end{flushright}}
\newcommand{\trans}{^{\mbox{\tiny{T}}}}
%\newcommand{\trans}{\top}
\newcommand{\T}{\trans}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special reliability analysis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nc{\h}{\mbox{$h(\bmp)$}}
\nc{\hm}{\mbox{$h^m(\bmp)$}}
\nc{\hnei}{\mbox{$h({\bf p})$}}
\nc{\hmnei}{\mbox{$h^m({\bf p})$}}
\nc{\hj}{h_j(\bmp)}
\nc{\hmj}{h_j^m(\bmp)}
\nc{\hjm}{\hmj}
\nc{\ph}{\phi(\bmx)}
\nc{\Ph}{\phi(\bmX)}
%\nc{\p}{\overline P}
\nc{\ip}{\coprod}
\nc{\phd}{\phi^D (\bmx)}
\nc{\Phd}{\phi^D(\bmX)}
\nc{\hd}{h^D (\bmp)}
\nc{\hdm}{\left( h^D (\bmp) \right)^m}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BN related stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \nc{\pa}[1]{{\rm pa}\left(#1\right)}
 \nc{\mb}[1]{{\rm mb}\left(#1\right)}
 \nc{\sspace}[1]{\ensuremath{sp\left(#1\right)}}
% \nc{\sspace}[1]{{\rm sp}\left(#1\right)}
 \nc{\child}[1]{\mbox{${\rm ch}\left(#1\right)$}}
 \nc{\indep}{\mbox{$\perp\!\!\!\perp$}}
 \nc{\nonindep}{\not\!\!\!\indep} \nc{\NB}{Na\"{\i}ve Bayes\xspace}
 \nc{\nB}{na\"{\i}ve Bayes\xspace}
 \nc{\MDL}{\mbox{MDL}\xspace} \nc{\MDLp}{$\mbox{MDL}_p$\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This part here for the HuginToPsTrics stuff by Thomas
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Fbox}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\parbox[c][#1]{#1}{\centerline{#5}}}}}}
\newcommand{\Fnode}[5][0.5cm]{\cnodeput[doubleline=false](#2,#3){#4}{\makebox[#1]{#5}}}
\newcommand{\FDblnode}[5][0.5cm]{\cnodeput[doubleline=true](#2,#3){#4}{\makebox[#1]{#5}}}
\newcommand{\Fdiam}[5][0.3cm]{\rput(#2,#3){\dianode{#4}{\makebox[#1]{#5}}}}
\newcommand{\Fovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode{#4}{\makebox[#1]{#5}}}}
\newcommand{\FDblovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode[doubleline=true]{#4}{\makebox[#1]{#5}}}}
\newcommand{\Frect}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\makebox[#1]{#5}}}}}
\newcommand{\arc}[3][solid]{\ncline[linestyle=#1]{->}{#2}{#3}}
%\newpsobject{showgrid}{psgrid}{subgriddiv=1,griddots=10,gridlabels=6pt}
%\psset{unit=0.5cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% pstexfig: Latex-type figures from xfig.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\pstexfig}[2] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \input{./FIGS/#1.pstex_t}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}

\newcommand{\pstexFig}[2] {
\begin{nopagebreak}
  \begin{figure*}[htbp]
    \begin{center}
      \input{./FIGS/#1.pstex_t}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure*}
\end{nopagebreak}
}

\newcommand{\pstexfigSlide}[1] {
\begin{nopagebreak}
    \begin{center}
        \input{./#1.pstex_t}
    \end{center}
\end{nopagebreak}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% epsfigur: Get an eps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\epsfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \epsfig{file =./FIGS/#1.eps,width=#3mm}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% psfigur: Get an ps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\psfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \psfig{file =./FIGS/#1.ps,width=#3mm,angle=-90}
       \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Rpsfigur: Get an ps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Rpsfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \psfig{file =./FIGS/#1.ps,width=#3mm}
       \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}



\nc{\figref}[1]{\figurename~\ref{fig:#1}\xspace}
\nc{\tabref}[1]{Table~\ref{tab:#1}\xspace}
\nc{\equref}[1]{Equation~(\ref{equ:#1})\xspace}
\nc{\secref}[1]{Section~\ref{sec:#1}\xspace}
\nc{\algoref}[1]{Algorithm~\ref{algo:#1}\xspace}
\nc{\stepref}[1]{Step~\ref{step:#1}\xspace}

\nc{\includebib}{\bibliography{defs,%
                               hl,%
                               master,%
                               dynamic,%
                               reliability,%
                               troubleshoot,%
                               class,%
                               learning,%
                               luigi,%
			      footy,%
                               antonio,%
%                               mte,%
                               global%
}}


==> misc.tex <==



% https://math.stackexchange.com/questions/840855/inverse-of-constant-matrix-plus-diagonal-matrix



\section{Lower bound for variance}
Let \(g(\bmtheta) = f(y, \bmx; \bmtheta)\), and \(\bmtheta \sim =\rho(\bmtheta;p) = Binom(1, p)\). Then

Hypothesis:
\[
    \E_{\rho}\left[ \frac{\partial}{\partial p} \log \rho(\bmtheta;p) \right] = 0
\]
Then 
\begin{align*}
        a(p) &= \E_{\rho} \left[ g(\bmtheta) \frac{\partial}{\partial p} \log \rho(\bmtheta;p) \right]\\
        &= p g(\bmtheta_1) \frac{\partial}{\partial p} \log \rho(\bmtheta_1;p) + (1-p) g(\bmtheta_2) \frac{\partial}{\partial p} \log \rho(\bmtheta_2;p)\\
        &= p g(\bmtheta_1) \frac{\partial}{\partial p} \log p + (1-p) g(\bmtheta_2) \frac{\partial}{\partial p} \log (1-p)\\
        &= g(\bmtheta_1) - g(\bmtheta_2) \\
        &= f(y, \bmx; \bmtheta_1) - f(y, \bmx; \bmtheta_2)
\end{align*}

\[
    \V[f(y, \bmx; \bmtheta)] \geq \frac{a(p)^2}{nJ(p)}
\]
\[
    J(p) = \E_\rho\left[ \left(\frac{\partial}{\partial p}\log \rho(\bmtheta; p)\right)^2\right]
\]
\begin{align*}
    J(p) &= p \left(\frac{\partial}{\partial p}\log p\right)^2 + (1- p) \left(\frac{\partial}{\partial p}(1-p)\right)^2\\
    &= \frac{1}{p}+ \frac{1}{1-p} = \frac{1}{p(1-p)} = n\V_\rho[\bmtheta]^{-1}
\end{align*}
\[
 \V_\rho[f(y, \bmx; \bmtheta)] \geq \frac{a(p)^2}{nJ(p)} = \V_\rho[\bmtheta]( f(y, \bmx; \bmtheta_1) - f(y, \bmx; \bmtheta_2))^2
\]

Multinomial: \(\bmtheta \sim Multinomial(1, \bm{p})\) with \(\bm p = (p_1, \dots, p_{k-1}, 1-p_1-\dots-p_{k-1})\)
\begin{align*}
        a_i(p) &= \E_{\rho(\bmtheta;p)} \left[ g(\bmtheta) \frac{\partial}{\partial p_i} \log \rho(\bmtheta;p) \right]\\
        &=\sum_{j=1}^{K}\rho(\bmtheta_j;p)g(\bmtheta_j) \frac{\partial}{\partial p_i} \log \rho(\bmtheta_j;p)\\
         &=\sum_{j=1}^{K-1}p_j g(\bmtheta_j) \frac{\partial}{\partial p_i} \log p_j\\
         &+ (1-\sum_j p_j) g(\bmtheta_{K}) \frac{\partial}{\partial p_i} \log (1-\sum_j p_j)\\
         &= g(\bmtheta_i)-g(\bmtheta_K)
\end{align*}

\[a(p) = \frac{\partial}{\partial p} \E_{\rho(\bmtheta;p)}[ g(\bmtheta)]\]

\[
 \V_\rho[f(y, \bmx; \bmtheta)] \geq a(p)^T J(p)^{-1}a(p)
\]

\begin{align*}
J_{i,j}(p) &= \E_{\rho(\bmtheta;p)} \left[ \frac{\partial \log \rho(\bmtheta;p)}{\partial p_i \partial p_j}\right]\\
&= \sum_{m=1}^{K-1} p_m \frac{\partial \log \rho(\bmtheta_m;p)}{\partial p_i \partial p_j}\\
&+ (1-\sum_m p_m) \frac{\partial \log \rho(\bmtheta_K;p)}{\partial p_i \partial p_j} \\
\end{align*}
\[
    \frac{\partial \log \rho(\bmtheta_K;p)}{\partial p_i} =\frac{\partial}{\partial p_i} \log(1 - \sum_m p_m) = \frac{-1}{1 - \sum_m p_m}
\]
\[
    \frac{\partial^2 \log \rho(\bmtheta_K;p)}{\partial p_i p_j} =(-1)\frac{\partial}{\partial p_j} (1 - \sum_m p_m)^{-1} = (-1)(1 - \sum_m p_m)^{-2}
\]
\[
    J_{i,j\neq i}(p) = (-1)(1 - \sum_{m=1}^{k-1} p_m)^{-1}
\]
\[
    J_{i,i}(p) = (-1)(1 - \sum_{m=1}^{k-1} p_m)^{-1} - \frac{1}{p_i^2}
\]

\[
    J_{i,j\neq i}(p) = (\sum_{m=1}^{k-1} p_m - 1)^{-1}
\]

\[
    J_{i,i}(p) = (\sum_{m=1}^{k-1} p_m-1)^{-1} \big(1- \frac{(\sum_{m=1}^{k-1} p_m-1)}{p_i^2}\big)
\]

\[ J = q1 + q diag(\frac{1}{p_i^2})\]

\[
 \V_\rho[f(y, \bmx; \bmtheta)] \geq \V_\rho[\bmtheta]\sum_i (f(y, \bmx; \bmtheta_i) - f(y, \bmx; \bmtheta_K))^2
\]




\subsection{How to Exploit Diversity to Learn Ensembles?}
\label{sec:diversity:learning}

The PAC-Bayesian bounds of Theorem \ref{thm:2ndPACBayes} provide a sound framework for ensemble learning. As they simultaneously hold for all distributions $\rho$, we can choose the distribution $\rho$ which minimizes these high-probability upper-bounds over the generalization error of the ensemble \citep{GLL+15,masegosa2020learning,masegosa2020second}. 


However, ensembles of neural networks are parametrized in highly dimensional continuous parameter spaces and, so far, we have been considering that the parameter space $\bmTheta$ is defined by a finite set of parameters\footnote{See the discussion given at Appendix~\ref{app:4.4} to see that, in any case, this is a fairly general setting.}. Given this learning task, we need to consider that $\bmTheta\subseteq \Re^M$ and, in consequence,  both $\rho$ and $\pi$ should be now density functions over $\bmTheta$. Fortunately, as we show in Appendix~\ref{app:4.4}, all previous results, including the PAC-Bayesian bounds of Theorem \ref{thm:2ndPACBayes}, hold either for a continuous or a finite parameter space. In this appendix we also show, using a similar approach to \citep{masegosa2020learning}, 


In Appendix~\ref{app:4.4}, 

We follow a similar approach to \citep{masegosa2020learning} and employ an uniform mixture of $K$ multivariate Gaussian distributions, denoted as $\rho_\delta$, to represent an ensemble of $K$ models. The means of the $K$ components of the mixture are defined by $K$ parameters $\{\bmtheta_1,\ldots,\bmtheta_K\}$ and all the Gaussian distributions have a diagonal covarariance matrix defined by a fixed and small scalar $\epsilon>0$ (i.e. $\Sigma=\epsilon I$). By fixing $\lambda=2$ and discarding constant terms, the minimization of the PAC-Bayesian bound of Theorem \ref{thm:2ndPACBayes} can be jointly as follows, 
\begin{equation}\label{eq:PACLearning}
 \rho^\star_\delta = \arg \min_{\rho_\delta} \E_{\rho_\delta}[\hat{L}(\bmtheta,D)] - \hat{V}({\rho_\delta},D) + \frac{2\kl{\rho_\delta}{\pi}}{n},
\end{equation}
\noindent where $\kl{\rho_\delta}{\pi}$ acts as a regularizer and we fixed the hyperparameter $\lambda$ to 1. In Appendix~\ref{app:4.4}, we show that, for a sufficiently small $\epsilon>0$, the rhs of the above equation can be simplified with the following approximations\footnote{Because $\rho_\delta$ can be approximated by an uniform mixture of Dirac delta distributions.}: $\E_{\rho_\delta}[\hat{L}(\bmtheta,D)]\approx\frac{1}{K}\sum_i\hat{L}(\bmtheta_i,D)$,  $\hat{V}({\rho_\delta},D)$ and $\kl{\rho_\delta}{\pi}\approx -\frac{1}{K}\sum_i \ln \pi(\bmtheta_i) + C$ where $C$ is a positive constant. As a result, the learning problem is reduced to determining the $K$ parameters $\{\bmtheta_1,\ldots,\bmtheta_K\}$ that minimize Equation \eqref{eq:PACLearning}. This learning approach was proposed by \citep{masegosa2020learning} in the context of the cross-entropy loss and the $\CE$-version of the PAC-Bayesian bound of Theorem \ref{thm:2ndPACBayes}. Here, we show that it can be extended to other kind of ensembles. 
%
%
%
%In order to deal with the problem of ensemble learning in continuous spaces, we rep
%
%In this case, we follow \citep{masegosa2020learning}, and employ uniform mixtures of Dirac-delta distributions, denoted as $\rho_\delta$, parametrized by a set of $K$ parameters $\{\bmtheta_1,\ldots,\bmtheta_K\}$ to represent any ensemble of $K$ models. So, as shown in \citep{masegosa2020learning}, an ensemble learning method based on the minimization of the continuous extensions of the PAC-Bayesian bounds of Theorem \ref{thm:2ndPACBayes} can be approximated by the following minimization problem,
%\begin{equation}\label{eq:PACLearning}
% \rho^\star_\delta = \arg \min_{\rho_\delta} \E_{\rho_\delta}[\hat{L}(\bmtheta,D)] - \hat{V}({\rho_\delta},D) + \frac{2\E_{\rho_\delta}[\ln \pi(\bmtheta)]}{\lambda n}
%\end{equation}
%\noindent where, by standard properties of Dirac-delta distributions, $\E_{\rho_\delta}[\hat{L}(\bmtheta,D)]=\frac{1}{K}\sum_i\hat{L}(\bmtheta_i,D)$, $\E_{\rho_\delta}[\ln \pi(\bmtheta)]=\frac{1}{K}\sum_i \ln \pi(\bmtheta_i)$ and, similarly, for the $\hat{V}({\rho_\delta},D)$ term. This minimization problem over $\rho_\delta$ is equivalent to a minimization problem over $\{\bmtheta_1,\ldots,\bmtheta_K\}$ and, in consequence, the distribution $\rho^\star_\delta$ will define the learned ensemble. Full details of this derivation are given in Appendix ?. In this case, we only consider for the above equation the mean-square-error and the cross-entropy loss, because the 0-1 loss is non differentiable. 

Equation \eqref{eq:PACLearning} shows how we can exploit diversity to learn an ensemble: we should find models with small empirical loss ($\E_{\rho_\delta}[\hat{L}(\bmtheta,D)]$), high empirical variance ($\hat{V}(\rho,D)$) and small regularization $\kl{\rho_\delta}{\pi}$. Moreover, Equation \eqref{eq:PACLearning} provides a theoretical framework to understand the rationale behind many learning algorithms for neural network ensembles present in the literature. 

As discussed in Section \ref{sec:rw}, a growing number of ensemble learning approaches \citep{liu1999ensemble,jiang2017generalized,buschjager2020generalized} employs learning objectives which, besides the $\E_{\rho_\delta}[\hat{L}(\bmtheta,D)]$ term and a regularizer, also include a term which explicitly encourages diversity. Except for \citep{krogh1995validation}, who employs $\hat{V}_{\MSE}({\rho_\delta},D)$ for this purpose. The diversity-promoting terms considered in these works do not match the variance $\hat{V}({\rho_\delta},D)$ term, but they are related. In consequence, Equation \eqref{eq:PACLearning}  provides a clear theoretical justification of these diversity-promoting approaches as they can be described as ensemble learning methods that (approximately) minimize a high-probability upper-bound over the generalization error of the ensemble. More details of this analysis can be found in Appendix \ref{app:4.4}. 


%Equation \eqref{eq:PACLearning} shows how we can exploit diversity to learn an ensemble: we should find models with small empirical loss (i.e., $\E_{\rho_\delta}[\hat{L}(\bmtheta)]$), high empirical variance (i.e., $\hat{V}(\rho,D)$) and small regularization error $\kl{\rho_\delta}{\pi}$.  In the literature there are two different set of approaches to achieve this goal in the context of ensembles of neural networks.  A growing set of approaches [18][...] minimizes learning objectives which, besides the $\E_{\rho_\delta}[\hat{L}(\bmtheta,D)]$ and $\E_{\rho_\delta}[\ln \pi(\bmtheta)]$ terms, include a term which explicitly encourages diversity. Although these works do not explicitly include the $ \hat{V}({\rho_\delta},D)$ term for encouraging diversity, they employ terms which are related. In consequence, this work provides a clear theoretical explanation of the rationale of these approaches. In Appendix ?, we provide detail discussions for each one of these approaches. 

The most popular approaches \citep{lakshminarayanan2017simple,wen2019batchensemble,wenzel2020hyperparameter} are based on minimizing a learning objective which only considers the expected loss $\E_{\rho_\delta}[\hat{L}(\bmtheta,D)]$ plus a regularizing term. Consequently, they do not explicitly include a term which encourages diversity. However, these methods exploit the multi-modality of the loss's landscape of neural networks \citep{fort2019deep} to promote diversity. More precisely, they induce the individual models to converge to different modes of the learning objective. E.g., \citep{lakshminarayanan2017simple,wen2019batchensemble} employ random initializations to force the gradient descent method to converge to different local minima, while \citep{wenzel2020hyperparameter} additionally apply different hyperparameter configurations to achieve this goal. As we show in Appendix~\ref{app:4.4}, these ensemble learning approaches are minimizing $\E_{\rho_\delta}[\hat{L}(\bmtheta,D)] + \frac{\kl{\rho_\delta}{\pi}}{n}$, and, if each local minima defines a different function (i.e., $h(\cdot,\bmtheta_i)\neq h(\cdot,\bmtheta_j)$ if $i\neq j$) as usually happens in neural networks \citep{li2017visualizing,fort2019deep}, we end up with a solution where $\hat{V}(\rho^\star_\delta,D)>0$. Our experimental evaluation, but also the results reported in any of these works, show that this strategy can be quite effective to jointly minimize the average empirical loss of individual models while having a high degree of diversity among them, specially in the presence of highly multi-modal parameter spaces. In that sense, this work provides a clear theoretical explanation of the rationale beside these ensemble learning approaches. 

%More precisely, this minimization problem of Equation \eqref{eq:PACLearning} can be decomposed in independent minimization problems: $\bmtheta_i^\star = \arg\min_{\bmtheta_i}\E_{\rho_\delta}[\hat{L}(\bmtheta,D)] + \E_{\rho_\delta}[\ln\pi(\bmtheta)]=\arg\min_{\bmtheta_i} \hat{L}(\bmtheta_i,D) + R(\bmtheta_i)$, and it is well known that $\hat{L}(\bmtheta_i,D)$ is a multi-modal function in the case of neural networks and the cross-entropy or the mean-square-error loss []. Different methods exploit different strategies to find $\bmtheta_i^\star$ which are local opitma. E.g., \citep{lakshminarayanan2017simple,wen2019batchensemble} employ random initializations to force the gradient descent method to converge to different local minima, while \citep{wenzel2020hyperparameter} additionally applies different hyperparameter configurations to achieve this goal too. 

